A Program Logic to Verify Signal Temporal Logic Specifications of Hybrid Systems: Extended Technical Report

Signal temporal logic (STL) was introduced for monitoring temporal properties of continuous-time signals for continuous and hybrid systems. Differential dynamic logic (dL) was introduced to reason about the end states of a hybrid program. Over the past decade, STL and its variants have significantly gained in popularity in the industry for monitoring purposes, while dL has gained in popularity for verification of hybrid systems. In this paper, we bridge the gap between the two different logics by introducing signal temporal dynamic logic (STdL) -- a dynamic logic that reasons about a subset of STL specifications over executions of hybrid systems. Our work demonstrates that STL can be used for deductive verification of hybrid systems. STdL significantly augments the expressiveness of dL by allowing reasoning about temporal properties in given time intervals. We provide a semantics and a proof calculus for STdL, along with a proof of soundness and relative completeness.

==> casestudy.tex <==
\section{Case Study: Traction Assist in Automobiles}\label{sec:casestudy}
In this section, we go over a simplified case study for \stdl inspired by the industry to show its power for unbounded verification purposes. Consider a car with accelerator (or throttle) input $\omega$ cruising on the road, with a signal ${\sf no\_traction}$ that streams a binary value of ${\sf true}$ or ${\sf false}$ corresponding to whether or not the car's sensors detect that the car is skidding or losing traction and a boolean flag ${\sf traction\_control}$ corresponding to whether or not the vehicle's traction control is engaged. The accelerator input $\omega$ can have a positive or negative value corresponding to acceleration and deceleration respectively, or a value of zero corresponding to no acceleration. The wheel rotation $\rho$ of the car's wheels evolves according to differential equation 
$${\sf cruise}(\omega) ::= \rho' = \omega \times k - \varphi \times j$$ 
for some constants $k$ and $j$, where $\varphi$ represents the braking force applied to the car's wheels.\footnote{In practice, each of the car's wheels could have a different wheel rotation and braking force. For the sake of simplicity, and to avoid presenting four separate proofs in this case study, we assume that each wheel has the same rotation and braking force.} Let there be a safety property $\phi$ requiring that in the event that the car is skidding, a vehicle traction assist program executes to help gain traction again and slow down the wheel spin to stop the skidding, following which the car can accelerate again. According to the safety property, after running the traction assist program, the car's traction control should turn on and within 1 to 5 seconds, the car's wheel rotation $\rho$ should fall to under some constant $\rho_0$ (to help regain control). 

A very simple version of the hybrid program ${\sf traction\_assist}$ can then take the form:
\begin{align}
    {\sf traction\_assist} ::=&\ ( ?({\sf no\_traction}); \\
    &\ {\sf traction\_control := 1};\\ 
    &\ \omega := -1;\ \rho' = {\sf cruise(\omega)});
\end{align}
Several properties of hybrid programs are present in ${\sf traction\_assist}$. (1) denotes a test to check whether the car has lost traction; (2) represents an assignment statement setting ${\sf traction\_control}$ to on; and (3) shows an evolving ordinary differential equation that changes the wheel rotation of the car. The sequential composition operator joins the individual statements together to form a single hybrid program.
%\hammad{TODO: Anti-lock braking system makes you release the brake until traction is regained, and then applies the brakes again. (look at Wikipedia ABS article). look at STL case studies (papers that cite the STL papers), try to get some inspiration from there by looking at differential equations. (suitable conferences include EMSOFT, HSCC, NFM, iFM, FM, etc...)}
The safety property $\phi$ described above can be expressed as:
$$\phi ::= {\sf \boxp{traction\_assist}} 
\left(
\begin{tabular}{c}
    $\lnot{\sf no\_traction}$ $\sqor$ $\dia_{[1, 5]}(\rho < \rho_0)$
\end{tabular}
\right)$$
We present a proof sketch of this safety property in Appendix~\ref{appendix:casestudy}. Safety properties of this type are expressible in \stdl (but, to the best of our knowledge, not in any other logic preceding \stdl). This case study shows how \stdl can be used to ensure that some property holds in a given time interval during the execution of a hybrid program, thereby enabling verification of crucial safety and liveness properties of hybrid systems. 

